Breaking Barriers in Physical-World Adversarial Examples: Improving Robustness and Transferability via Robust Feature

As deep neural networks (DNNs) are widely applied in the physical world, many researches are focusing on physical-world adversarial examples (PAEs), which introduce perturbations to inputs and cause the model's incorrect outputs. However, existing PAEs face two challenges: unsatisfactory attack performance (i.e., poor transferability and insufficient robustness to environment conditions), and difficulty in balancing attack effectiveness with stealthiness, where better attack effectiveness often makes PAEs more perceptible. In this paper, we explore a novel perturbation-based method to overcome the challenges. For the first challenge, we introduce a strategy Deceptive RF injection based on robust features (RFs) that are predictive, robust to perturbations, and consistent across different models. Specifically, it improves the transferability and robustness of PAEs by covering RFs of other classes onto the predictive features in clean images. For the second challenge, we introduce another strategy Adversarial Semantic Pattern Minimization, which removes most perturbations and retains only essential adversarial patterns in AEsBased on the two strategies, we design our method Robust Feature Coverage Attack (RFCoA), comprising Robust Feature Disentanglement and Adversarial Feature Fusion. In the first stage, we extract target class RFs in feature space. In the second stage, we use attention-based feature fusion to overlay these RFs onto predictive features of clean images and remove unnecessary perturbations. Experiments show our method's superior transferability, robustness, and stealthiness compared to existing state-of-the-art methods. Additionally, our method's effectiveness can extend to Large Vision-Language Models (LVLMs), indicating its potential applicability to more complex tasks.

==> Section/6-checklist.tex <==
\section*{Reproducibility Checklist}

% Unless specified otherwise, please answer “yes” to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled “Reproducibility Checklist” at the end of the technical appendix.


%  \answerYes{Yes}
% \answerNo{No}
% \answerNA{NA}

\begin{enumerate}

\item This paper:
\begin{enumerate}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced.
    \answerYes{Yes}
    \item Clearly delineates statements that are opinions, hypotheses, and speculation from objective facts and results.
    \answerYes{Yes}
    \item Provides well-marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper.
    \answerYes{Yes}
\end{enumerate}

\item Does this paper make theoretical contributions?
\begin{enumerate}
    \item All assumptions and restrictions are stated clearly and formally.
    \answerYes{Yes}
    \item All novel claims are stated formally (e.g., in theorem statements).
    \answerYes{Yes}
    \item Proofs of all novel claims are included.
    \answerYes{Yes}
    \item Proof sketches or intuitions are given for complex and/or novel results.
   \answerYes{Yes}
    \item Appropriate citations to theoretical tools used are given.
    \answerYes{Yes}
    \item All theoretical claims are demonstrated empirically to hold.
    \answerYes{Yes}
    \item All experimental code used to eliminate or disprove claims is included.
     \answerNA{NA}
\end{enumerate}

\item Does this paper rely on one or more datasets?
\begin{enumerate}
    \item A motivation is given for why the experiments are conducted on the selected datasets.
    \answerYes{Yes}
    \item All novel datasets introduced in this paper are included in a data appendix.
    \answerNA{NA}
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes.
    \answerNA{NA}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations.
    \answerYes{Yes}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available.
    \answerYes{Yes}
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisfying.
    \answerNA{NA}
\end{enumerate}

\item Does this paper include computational experiments?
\begin{enumerate}
    \item Any code required for pre-processing data is included in the appendix.
     \answerYes{Yes}
    \item All source code required for conducting and analyzing the experiments is included in a code appendix.
     \answerYes{Yes}
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes.
     \answerYes{Yes}
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from.
     \answerYes{Yes}
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results.
     \answerYes{Yes}
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks.
     \answerYes{Yes}
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics.
    \answerYes{Yes}
    \item This paper states the number of algorithm runs used to compute each reported result.
     \answerYes{Yes}
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information.
     \answerYes{Yes}
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank).
    \answerYes{Yes}
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments.
    \answerYes{Yes}
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting.
    \answerYes{Yes}
\end{enumerate}

\end{enumerate}


